Efficient Parameterized Pattern Matching in Sublinear Space

The parameterized matching problem is a variant of string matching, which is to search for all parameterized occurrences of a pattern $P$ in a text $T$. In considering matching algorithms, the combinatorial natures of strings, especially periodicity, play an important role. In this paper, we analyze the properties of periods of parameterized strings and propose a generalization of Galil and Seiferas's exact matching algorithm (1980) into parameterized matching, which runs in $O(\pi|T|+|P|)$ time and $O(\log{|P|}+|{\rm\Pi}|)$ space in addition to the input space, where ${\rm\Pi}$ is the parameter alphabet and $\pi$ is the number of parameter characters appearing in $P$ plus one.

==> docs/acknowledgements.tex <==
\subsubsection*{Acknowledgements}
The authors deeply appreciate the anonymous reviewers helpful comments.
This work was supported by JSPS KAKENHI Grant Numbers JP19K20208 (DH), JP18H04091 (RY), JP18K11150 (RY), JP19K12098 (RY), JP20H05703 (RY), and JP21K11745 (AS).

